Intrinsic Task-based Evaluation for Referring Expression Generation

Recently, a human evaluation study of Referring Expression Generation (REG) models had an unexpected conclusion: on \textsc{webnlg}, Referring Expressions (REs) generated by the state-of-the-art neural models were not only indistinguishable from the REs in \textsc{webnlg} but also from the REs generated by a simple rule-based system. Here, we argue that this limitation could stem from the use of a purely ratings-based human evaluation (which is a common practice in Natural Language Generation). To investigate these issues, we propose an intrinsic task-based evaluation for REG models, in which, in addition to rating the quality of REs, participants were asked to accomplish two meta-level tasks. One of these tasks concerns the referential success of each RE; the other task asks participants to suggest a better alternative for each RE. The outcomes suggest that, in comparison to previous evaluations, the new evaluation protocol assesses the performance of each REG model more comprehensively and makes the participants' ratings more reliable and discriminable.

==> sec/hypothesis.tex <==
\section{Hypotheses} \label{sec:hypo}

\input{tab/successful_results}

Based on our research questions and related discussions in Section~\ref{sec:rq}, we have the following hypotheses.

% KvD I'm a bit unclear about our hypotheses and RQs:
%-- Has each Hyp been tested statistically? (I couldn't see that in the case of H1 and H2.
%-- Are these RQs and Hyp's all independent of each other? (It seems to me that our key RQ1 and the more low-level RQ3 are closely related.) Should a Bonferroni correction be performed? Alternatively, should we make it clear that RQ1 is key, and the rest is more like houskeeping?
% -- It's not super easy to spot the fate of each hypothesis, for example because they're discussed in a different order than the one in which they were introduced (and numbered). 

\paragraph{Hypothesis 1 ($\mathcal{H}_1$)} The meta-level tasks help participants make more informed ratings. Therefore, unlike the findings by~\citet{same-etal-2022-non}, we expect to observe significant distinguishable differences in the overall ratings of the models. 

\paragraph{Hypothesis 2 ($\mathcal{H}_2$)} Since the tasks help participants identify inappropriate REs in each discourse, we expected that the scores in this experiment would be lower than those in~\citet{same-etal-2022-non}.

\paragraph{Hypothesis 3 ($\mathcal{H}_3$)} Regarding the successfulness of REs, we expected that the more frequently REs are marked as successful, the higher the discourse would be rated.

\paragraph{Hypothesis 4 ($\mathcal{H}_4$)} We expected that the more often the REs are re-written, the lower the scores the discourse would receive. 

\paragraph{Hypothesis 5 ($\mathcal{H}_5$)} We expected that participants would spot more inappropriate REs in discourse if they were familiar with its major entity and, as a consequence, they would re-write more and rate the discourse lower.
